An Approach to "Quantumness" in Coherent Control

Developments in the foundations of quantum mechanics have identified several attributes and tests associated with the "quantumness" of systems, including entanglement, nonlocality, quantum erasure, Bell test, etc. Here we introduce and utilize these tools to examine the role of quantum coherence and nonclassical effects in 1 vs. N photon coherent phase control, a paradigm for an all-optical method for manipulating molecular dynamics. In addition, truly quantum control scenarios are introduced and examined. The approach adopted here serves as a template for studies of the role of quantum mechanics in other coherent control and optimal control scenarios.

==> pgfsettings.tex <==
\usetikzlibrary{calc,shapes,shapes.callouts,decorations.markings,arrows,patterns,chains,matrix,positioning,automata,scopes,spy}

\usetikzlibrary{external}
\tikzexternalize[mode=list and make,prefix=./]
\tikzset{external/system call={pdflatex \tikzexternalcheckshellescape -interaction=batchmode -jobname "\image" "\texsource"}}
\tikzexternaldisable

\RequirePackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots,polar}

\tikzstyle{ultra thin}=[line width=.0375ex]
\tikzstyle{very thin}=[line width=.075ex]
\tikzstyle{thin}=[line width=.15ex]
\tikzstyle{semithick}=[line width=0.225ex]
\tikzstyle{thick}=[line width=.3ex]
\tikzstyle{very thick}=[line width=.375ex]
\tikzstyle{ultra thick}=[line width=.45ex]

\tikzstyle{solid}=[dash pattern=]
\tikzstyle{dotted}=[dash pattern=on \pgflinewidth off 4\pgflinewidth]
\tikzstyle{densely dotted}=[dash pattern=on \pgflinewidth off 2\pgflinewidth]
\tikzstyle{loosely dotted}=[dash pattern=on \pgflinewidth off 8\pgflinewidth]
\tikzstyle{dashed}=[dash pattern=on 6\pgflinewidth off 6\pgflinewidth]
\tikzstyle{densely dashed}=[dash pattern=on 6\pgflinewidth off 4\pgflinewidth]
\tikzstyle{loosely dashed}=[dash pattern=on 6\pgflinewidth off 12\pgflinewidth]
\tikzstyle{dot-dashed}=[dash pattern=on \pgflinewidth off 4\pgflinewidth on 6\pgflinewidth off 6\pgflinewidth]
\tikzstyle{densely dot-dashed}=[dash pattern=on \pgflinewidth off 2\pgflinewidth on 6\pgflinewidth off 4\pgflinewidth]
\tikzstyle{loosely dot-dashed}=[dash pattern=on \pgflinewidth off 8\pgflinewidth on 6\pgflinewidth off 12\pgflinewidth]
\tikzstyle{dot-dot-dashed}=[dash pattern=on \pgflinewidth off 4\pgflinewidth on \pgflinewidth off 4\pgflinewidth on 6\pgflinewidth off 6\pgflinewidth]
\tikzstyle{dot-dash-dashed}=[dash pattern=on \pgflinewidth off 4\pgflinewidth on 6\pgflinewidth off 6\pgflinewidth on 6\pgflinewidth off 6\pgflinewidth]

\makeatletter%
\pgfdeclareshape{mirror}{%
  \inheritsavedanchors[from=diamond]%
  \inheritanchorborder[from=diamond]%
  \foreach \anchor in {north,north west,north east,center,west,east,mid,mid west,mid east,base,base west,base east,south,south west,south east}{\inheritanchor[from=diamond]{\anchor}}%
  %\inheritbackgroundpath[from=diamond]%
  \backgroundpath{%
    \pgf@process{\outernortheast}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@xc by-1.414213\pgf@xa%
    \advance\pgf@yc by-1.414213\pgf@ya%
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgf@yc}}%
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgf@yc}}%
    \pgfpathclose%
  }%
}%
\pgfdeclareshape{beamsplitter}{%
  \inheritsavedanchors[from=diamond]%
  \inheritanchorborder[from=diamond]%
  \foreach \anchor in {north,north west,north east,center,west,east,mid,mid west,mid east,base,base west,base east,south,south west,south east}{\inheritanchor[from=diamond]{\anchor}}%
  %\inheritbackgroundpath[from=diamond]
  \backgroundpath{%
    \pgf@process{\outernortheast}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@xc by-1.414213\pgf@xa%
    \advance\pgf@yc by-1.414213\pgf@ya%
    \pgfpathmoveto{\pgfqpoint{0pt}{-\pgf@yc}}%
    \pgfpathlineto{\pgfqpoint{\pgf@xc}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{\pgf@yc}}%
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgf@yc}}%
    \pgfpathlineto{\pgfqpoint{-\pgf@xc}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{\pgf@yc}}%
    \pgfpathclose%
  }%
}%
\pgfdeclareshape{detector}{%
  \inheritsavedanchors[from=semicircle]%
  \inheritanchorborder[from=semicircle]%
  \foreach \anchor in {north,north west,north east,center,west,east,mid,mid west,mid east,base,base west,base east,south,south west,south east,apex,arc start,arc end,chord center}{\inheritanchor[from=semicircle]{\anchor}}%
  \inheritbackgroundpath[from=semicircle]%
}%
\pgfdeclareshape{phaseshifter}{%
  \inheritsavedanchors[from=circle]%
  \inheritanchorborder[from=circle]%
  \foreach \anchor in {north,north west,north east,center,west,east,mid,mid west,mid east,base,base west,base east,south,south west,south east}{\inheritanchor[from=circle]{\anchor}}%
  \inheritbackgroundpath[from=circle]%
  \beforebackgroundpath{%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xa<\pgf@ya%
      \advance\pgfutil@tempdima by-\pgf@ya%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xa%
    \fi%
    \advance\pgfutil@tempdima by-.5\pgflinewidth%
    \pgfsetshortenstart{0pt}%
    \pgfsetshortenend{0pt}%
    \pgfsetarrows{-}%
    \pgfpathmoveto{\pgfpointadd{\centerpoint}{\pgfqpoint{-0.7071\pgfutil@tempdima}{-0.7071\pgfutil@tempdima}}}%
    \pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpoint{0.7071\pgfutil@tempdima}{0.7071\pgfutil@tempdima}}}%
    \pgfusepath{stroke}%
    \pgfpathmoveto{\pgfpointadd{\centerpoint}{\pgfqpoint{0.7071\pgfutil@tempdima}{-0.7071\pgfutil@tempdima}}}%
    \pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpoint{-0.7071\pgfutil@tempdima}{0.7071\pgfutil@tempdima}}}%
    \pgfusepath{stroke}%
  }%
}%
\pgfdeclarepatternformonly{stripes}{\pgfpoint{0em}{0em}}{\pgfpoint{3em}{3em}}{\pgfpoint{3em}{3em}}
{
    \foreach \i in {0.3,0.9,1.5,2.1,2.7}
    {
     \pgfpathmoveto{\pgfpoint{\i em}{0em}}
     \pgfpathlineto{\pgfpoint{3em}{3em-\i em}}
     \pgfpathlineto{\pgfpoint{3em}{3em-\i em+0.3em}}
     \pgfpathlineto{\pgfpoint{\i em-0.3em}{0em}}
     \pgfpathclose%
     \pgfusepath{fill}
     \pgfpathmoveto{\pgfpoint{0em}{\i em}}
     \pgfpathlineto{\pgfpoint{3em-\i em}{3em}}
     \pgfpathlineto{\pgfpoint{3em-\i em-0.3em}{3em}}
     \pgfpathlineto{\pgfpoint{0em}{\i em+0.3em}}
     \pgfpathclose%
     \pgfusepath{fill}
    }
}
\makeatother%

\newdimen\XCoord
\newdimen\YCoord

